Generally-Altered, -Inflated, -Truncated and -Deflated Regression, With Application to Heaped and Seeped Data

Models such as the zero-inflated and zero-altered Poisson and zero-truncated binomial are well-established in modern regression analysis. We propose a super model that jointly and maximally unifies alteration, inflation, truncation and deflation for counts, given a 1- or 2-parameter parent (base) distribution. Seven disjoint sets of special value types are accommodated because all but truncation have parametric and nonparametric variants. Some highlights include: (i) the mixture distribution is exceeding flexible, e.g., up to seven modes; (ii) under-, equi- and over-dispersion can be handled using a negative binomial (NB) parent, with underdispersion handled by a novel Generally-Truncated-Expansion method; (iii) overdispersion can be studied holistically in terms of the four operators; (iv) an important application: heaped and seeped data from retrospective self-reported surveys are readily handled, e.g., spikes and dips which are located virtually anywhere; (v) while generally-altered regression explains why observations are there, generally-inflated regression accounts for why they are there in excess, and generally-deflated regression explains why observations are not there; (vi) the VGAM R package implements the methodology based on Fisher scoring and multinomial logit model (Poisson, NB, zeta and logarithmic parents are implemented.) The GAITD-NB has potential to become the Swiss army knife of count distributions.

==> pagelayout2.tex <==
% 20120111; pagelayout2.tex; for my book
% Has got extra colour stuff.



% 17/1/01;
% For distribution purposes, just toggle this


%% USA size; last modified 20090312
%  \oddsidemargin  -5mm       % USA 5mm?
%  \evensidemargin -5mm       % USA 5mm?
%  \headheight  8mm             % 10mm ok
%  \headsep   3mm              % was commented out before
% \textheight 240mm            % USA 240mm?
% \textwidth 160mm             % USA 160mm?
% \topmargin -10mm              % before 18/5/93 this was -20mm
% \topskip   2mm


% A4 paper
% ross suggested these be commented out
  \oddsidemargin  -10mm       % USA 5mm?
  \evensidemargin -10mm       % USA 5mm?
  \headheight 0mm             % 10mm ok
  \headsep  -3mm              % was commented out before
 \textheight 240mm            % USA 240mm? 250mm?
 \textwidth 180mm             % USA 160mm?
 \topmargin -4mm           % before 18/5/93 this was -20mm
 \topskip -10mm




% Note: (20130131)
% \newcommand{\bix}{\mbox{$\mathbf{\mathit{x}}$}}
% is italic but not bold.
% \newcommand{\bix}{\mbox{$\mathit{\mathbf{x}}$}}
% is not good.
% \newcommand{\bix}{\mbox{${\mathbf{x}}$}}
% seems the best.




% No longer needed because of BiBTeX
%\newcommand{\amerstat}[1]{{\em Amer.\ Statist.},\ {\bf #1}}
%\newcommand{\annstat}[1]{{\em Ann.\ Statist.},\ {\bf #1}}
%\newcommand{\appstat}[1]{{\em Appl.\ Statist.},\ {\bf #1}}
%\newcommand{\biometrika}[1]{{\em Biometrika},\ {\bf #1}}
%\newcommand{\biometrics}[1]{{\em Biometrics},\ {\bf #1}}
%\newcommand{\csda}[1]{{\em Comp.\ Statist.\ \&\ Data\ Analysis},
%\ {\bf #1}}
%\newcommand{\compstatda}[1]{{\em Comp.\ Statist.\ \&\ Data\ Analysis},
%\ {\bf #1}}
%\newcommand{\intstat}[1]{{\em Int.\ Statist.\ Review},\ {\bf #1}}
%\newcommand{\jappstat}[1]{{\em J.\ Appl.\ Statist.},\ {\bf #1}}
%\newcommand{\jasa}[1]{{\em J.\ Amer.\ Statist.\ Assoc.},\ {\bf #1}}
%\newcommand{\jcgs}[1]{{\em J.\ Comp.\ Graph.\ Statist.}, \ {\bf #1}}
%\newcommand{\jecon}[1]{{\em J.\ Econometrics},\ {\bf #1}}
%\newcommand{\jspi}[1]{{\em J.\ Statist.\ Plann.\ Inference.},\ {\bf #1}}
%\newcommand{\jrssa}[1]{{\em J.\ R.\ Statist.\ Soc.}\ A,\ {\bf #1}}
%\newcommand{\jrssb}[1]{{\em J.\ Roy.\ Statist.\ Soc.}\ B,\ {\bf #1}}
%\newcommand{\oz}[1]{{\em Austr.\ J.\ of Statist.},\ {\bf #1}}
%\newcommand{\sankhyaA}[1]{{\em Sankhya\ A},\ {\bf #1}}
%\newcommand{\science}[1]{{\em Science},\ {\bf #1}}
%\newcommand{\statcomp}[1]{{\em Statistics\ and Computing},\ {\bf #1}}
%%\newcommand{\statneer}[1]{{\em Statistica\ Neerlandica},\ {\bf #1}}
%\newcommand{\statneer}[1]{{\em Statist.\ Neerland.},\ {\bf #1}}
%\newcommand{\statsci}[1]{{\em Statist.\ Sci.},\ {\bf #1}}
%\newcommand{\statmed}[1]{{\em Statist.\ Med.},\ {\bf #1}}
%\newcommand{\tech}[1]{{\em Technomet.},\ {\bf #1}}
%\newcommand{\vegetatio}[1]{{\em Vegetatio},\ {\bf #1}}
%\newcommand{\jecol}[1]{{\em J.\ Ecol.},\ {\bf #1}}
%\newcommand{\ecology}[1]{{\em Ecology},\ {\bf #1}}
%\newcommand{\ecmon}[1]{{\em Ecol.\ Monogr.},\ {\bf #1}}


% the following comes from a Latex book p28
\newcommand{\namelistlabel}[1]{\mbox{#1}\hfil}
\newenvironment{namelist}[1]{%
\begin{list}{}
    {
      \let\makelabel\namelistlabel
      \settowidth{\labelwidth}{#1}
      \setlength{\leftmargin}{1.1\labelwidth}
    }
  }{%
\end{list}}

% Example:
% \begin{namelist}{XXXXXX}
% \item[{\sf Date:}]
%
% hello
% \end{namelist}


% For terms tests, assignments, etc.
\newcommand{\mk}[1]{\mbox{[1 mark]}}
\newcommand{\mks}[1]{\mbox{[#1 marks]}}


% 20100401; Good for copy-and-paste from .Rd files:
\newcommand{\code}[1]{\mbox{\texttt{\normalsize #1}}}
% \newcommand{\code}[1]{\mbox{\texttt{\small #1}}}



\newcommand{\convergeP}{\mbox{$\stackrel{\cal P}{\longrightarrow}$}}
\newcommand{\convergeD}{\mbox{$\stackrel{\cal D}{\longrightarrow}$}}
\newcommand{\convergeAS}{\mbox{$\stackrel{\rm a.s.}{\longrightarrow}$}}
\newcommand{\calA}{\mbox{${\cal A}$}}
\newcommand{\calB}{\mbox{${\cal B}$}}
\newcommand{\calC}{\mbox{${\cal C}$}}
\newcommand{\calD}{\mbox{${\cal D}$}}
\newcommand{\calF}{\mbox{${\cal F}$}}
\newcommand{\calH}{\mbox{${\cal H}$}}
\newcommand{\calI}{\mbox{${\cal I}$}}
\newcommand{\bcalI}{\mbox{\boldmath $\cal I$}}   % bold \cI
\newcommand{\calJ}{\mbox{${\cal J}$}}
\newcommand{\calj}{\mbox{${\cal j}$}}
\newcommand{\calL}{\mbox{${\cal L}$}}
\newcommand{\calLL}{\mbox{${\cal LL}$}}
\newcommand{\calAL}{\mbox{${\cal AL}$}}
\newcommand{\calM}{\mbox{${\cal M}$}}
\newcommand{\calN}{\mbox{${\cal N}$}}
\newcommand{\calP}{\mbox{${\cal P}$}}
\newcommand{\calR}{\mbox{${\cal R}$}}
\newcommand{\calS}{\mbox{${\cal S}$}}
\newcommand{\calT}{\mbox{${\cal T}$}}
\newcommand{\calV}{\mbox{${\cal V}$}}
\newcommand{\calW}{\mbox{${\cal W}$}}
\newcommand{\calX}{\mbox{${\cal X}$}}
\newcommand{\calY}{\mbox{${\cal Y}$}}
\newcommand{\scalA}{\mbox{\scriptsize ${\cal A}$}}
\newcommand{\scalI}{\mbox{\scriptsize ${\cal I}$}}
\newcommand{\scalD}{\mbox{\scriptsize ${\cal D}$}}
\newcommand{\scalM}{\mbox{\scriptsize ${\cal M}$}}
\newcommand{\scalR}{\mbox{\scriptsize ${\cal R}$}}
\newcommand{\scalS}{\mbox{\scriptsize ${\cal S}$}}
\newcommand{\scalT}{\mbox{\scriptsize ${\cal T}$}}
\newcommand{\scalX}{\mbox{\scriptsize ${\cal X}$}}
\newcommand{\scalY}{\mbox{\scriptsize ${\cal Y}$}}
\newcommand{\sbiX}{\mbox{\scriptsize \boldmath $X$}}
\newcommand{\sbix}{\mbox{\scriptsize \boldmath $x$}}
\newcommand{\bitX}{\mbox{\tiny \boldmath $X$}}
\newcommand{\bitx}{\mbox{\tiny \boldmath $x$}}
\newcommand{\sbiz}{\mbox{\scriptsize \boldmath $z$}}
\newcommand{\sbnu}{\mbox{\scriptsize \boldmath $\nu$}}
\newcommand{\stLM}{\mbox{\tiny  LM}}    % \tiny does not work for Biostatistics
\newcommand{\stVLM}{\mbox{\tiny VLM}}   % \tiny does not work for Biostatistics
\newcommand{\sformtwo}{\mbox{\scriptsize \tt form2}}
% \newcommand{\sformtwo}{\mbox{\scriptsize F2}}
\newcommand{\stPVLM}{\mbox{\tiny P-VLM}}




\def\ds{\displaystyle}

\newcommand{\bitY}{\mbox{\tiny \boldmath $Y$}}
\newcommand{\bity}{\mbox{\tiny \boldmath $y$}}
\newcommand{\sbiy}{\mbox{\scriptsize \boldmath $y$}}
\newcommand{\sbiY}{\mbox{\scriptsize \boldmath $Y$}}
\newcommand{\sbzero}{\mbox{\scriptsize \boldmath $0$}}
\newcommand{\sbomega}{\mbox{\scriptsize \boldmath $\omega$}}
\newcommand{\sbOmega}{\mbox{\scriptsize \boldmath $\Omega$}}
\newcommand{\sbalpha}{\mbox{\scriptsize \boldmath $\alpha$}}
\newcommand{\sbbeta}{\mbox{\scriptsize \boldmath $\beta$}}
\newcommand{\sbtheta}{\mbox{\scriptsize \boldmath $\theta$}}
\newcommand{\sbTheta}{\mbox{\scriptsize \boldmath $\Theta$}}
\newcommand{\Bin}{\mbox{\rm Binomial}}
\newcommand{\approxsim}{\mbox{$\stackrel{.}{\sim}$}}
\def\REAL{\hbox{\rm I \kern-5.5pt R}} % my alternative
\def\NAT{\hbox{\rm I \kern-5.5pt N}} % my alternative
%\def\SREAL{\mbox{\hbox{\rm \kern-2.5pt I \kern-2.5pt R}}} % my alternative
\def\SREAL{\mbox{{\footnotesize \hbox{\rm I \kern-3.5pt R}}}} % my alternative
\def\SNAT{\mbox{{\footnotesize \hbox{\rm I \kern-3.5pt N}}}} % my alternative

\newcommand{\pr}{\mbox{$P$}}
\newcommand{\cloglog}{\mbox{\rm cloglog}}
\newcommand{\logit}{\mbox{\rm logit}}
\newcommand{\rhobit}{\mbox{\rm rhobit}}
\newcommand{\bzero}{{\bf 0}}
\newcommand{\bone}{{\bf 1}}
\newcommand{\bc}{\mbox{\bf c}}
\newcommand{\bd}{\mbox{\bf d}}
\newcommand{\be}{\mbox{\bf e}}
\newcommand{\bh}{\mbox{\bf h}}
\newcommand{\bp}{\mbox{\bf p}}
\newcommand{\bu}{\mbox{\bf u}}
\newcommand{\bw}{\mbox{\bf w}}
\newcommand{\bx}{\mbox{\bf x}}


% 20130131; decommissioning these:
%\newcommand{\bia}{\mbox{\boldmath $a$}}
%\newcommand{\bib}{\mbox{\boldmath $b$}}
%\newcommand{\bic}{\mbox{\boldmath $c$}}
%\newcommand{\bid}{\mbox{\boldmath $d$}}
%\newcommand{\bie}{\mbox{\boldmath $e$}}
%\newcommand{\bif}{\mbox{\boldmath $f$}}
%\newcommand{\bolditg}{\mbox{\boldmath $g$}}
%\newcommand{\bih}{\mbox{\boldmath $h$}}
%\newcommand{\bolditn}{\mbox{\boldmath $n$}}
%\newcommand{\bim}{\mbox{\boldmath $m$}}
%\newcommand{\bio}{\mbox{\boldmath $o$}}
%\newcommand{\bip}{\mbox{\boldmath $p$}}
%\newcommand{\biq}{\mbox{\boldmath $q$}}
%\newcommand{\bir}{\mbox{\boldmath $r$}}
%\newcommand{\bis}{\mbox{\boldmath $s$}}
%\newcommand{\bit}{\mbox{\boldmath $t$}}
%\newcommand{\biu}{\mbox{\boldmath $u$}}
%\newcommand{\biv}{\mbox{\boldmath $v$}}
%\newcommand{\biw}{\mbox{\boldmath $w$}}
%%\newcommand{\bix}{\mbox{\boldmath $x$}}
%%\newcommand{\bix}{\mbox{$\mathbf{\mathit{x}}$}}
%\newcommand{\bix}{\mbox{$\mathbf{x}$}}
%\newcommand{\BIX}{\mbox{$\mathbf{X}$}}
%\newcommand{\biy}{\mbox{\boldmath $y$}}
%\newcommand{\biz}{\mbox{\boldmath $z$}}


% 20130131; commissioning these:
%\newcommand{\bia}{\mbox{$\mathbf{a}$}}
%\newcommand{\bib}{\mbox{$\mathbf{b}$}}
%\newcommand{\bic}{\mbox{$\mathbf{c}$}}
%\newcommand{\bid}{\mbox{$\mathbf{d}$}}
%\newcommand{\bie}{\mbox{$\mathbf{e}$}}
%\newcommand{\bif}{\mbox{$\mathbf{f}$}}
%\newcommand{\bolditg}{\mbox{$\mathbf{g}$}}
%\newcommand{\bih}{\mbox{$\mathbf{h}$}}
%\newcommand{\bolditn}{\mbox{$\mathbf{n}$}}
%\newcommand{\bim}{\mbox{$\mathbf{m}$}}
%\newcommand{\bio}{\mbox{$\mathbf{o}$}}
%\newcommand{\bip}{\mbox{$\mathbf{p}$}}
%\newcommand{\biq}{\mbox{$\mathbf{q}$}}
%\newcommand{\bir}{\mbox{$\mathbf{r}$}}
%\newcommand{\bis}{\mbox{$\mathbf{s}$}}
%\newcommand{\bit}{\mbox{$\mathbf{t}$}}
%\newcommand{\biu}{\mbox{$\mathbf{u}$}}
%\newcommand{\biv}{\mbox{$\mathbf{v}$}}
%\newcommand{\biw}{\mbox{$\mathbf{w}$}}
%\newcommand{\bix}{\mbox{$\mathbf{x}$}}
%\newcommand{\BIX}{\mbox{$\mathbf{x}$}}
%\newcommand{\biy}{\mbox{$\mathbf{y}$}}
%\newcommand{\biz}{\mbox{$\mathbf{z}$}}
%
%
%\newcommand{\biA}{\mbox{\boldmath $A$}}
%\newcommand{\biC}{\mbox{\boldmath $C$}}
%\newcommand{\biD}{\mbox{\boldmath $D$}}
%\newcommand{\biS}{\mbox{\boldmath $S$}}
%\newcommand{\biT}{\mbox{\boldmath $T$}}
%\newcommand{\biU}{\mbox{\boldmath $U$}}
%\newcommand{\biX}{\mbox{\boldmath $X$}}
%%\newcommand{\biY}{\mbox{\boldmath $Y$}}
%\newcommand{\biZ}{\mbox{\boldmath $Z$}}







% 20130926; inspired by Jakub. Needs \usepackage{bm}  in knitrheader.tex
\newcommand{\bia}{\mbox{$\bm{a}$}}
\newcommand{\bib}{\mbox{$\bm{b}$}}
\newcommand{\bic}{\mbox{$\bm{c}$}}
\newcommand{\bid}{\mbox{$\bm{d}$}}
\newcommand{\bie}{\mbox{$\bm{e}$}}
\newcommand{\bif}{\mbox{$\bm{f}$}}
\newcommand{\bolditg}{\mbox{$\bm{g}$}}
\newcommand{\bih}{\mbox{$\bm{h}$}}
\newcommand{\bolditi}{\mbox{$\bm{i}$}}
\newcommand{\bolditn}{\mbox{$\bm{n}$}}
\newcommand{\bim}{\mbox{$\bm{m}$}}
\newcommand{\bio}{\mbox{$\bm{o}$}}
\newcommand{\bip}{\mbox{$\bm{p}$}}
\newcommand{\biq}{\mbox{$\bm{q}$}}
\newcommand{\bir}{\mbox{$\bm{r}$}}
\newcommand{\bis}{\mbox{$\bm{s}$}}
\newcommand{\bit}{\mbox{$\bm{t}$}}
\newcommand{\biu}{\mbox{$\bm{u}$}}
\newcommand{\biv}{\mbox{$\bm{v}$}}
\newcommand{\biw}{\mbox{$\bm{w}$}}
\newcommand{\bix}{\mbox{$\bm{x}$}}
\newcommand{\BIX}{\mbox{$\bm{x}$}}
\newcommand{\biy}{\mbox{$\bm{y}$}}
\newcommand{\biz}{\mbox{$\bm{z}$}}


\newcommand{\biA}{\mbox{$\bm{A}$}}
\newcommand{\biC}{\mbox{$\bm{C}$}}
\newcommand{\biD}{\mbox{$\bm{D}$}}
\newcommand{\biP}{\mbox{$\bm{P}$}}
\newcommand{\biS}{\mbox{$\bm{S}$}}
\newcommand{\biT}{\mbox{$\bm{T}$}}
\newcommand{\biU}{\mbox{$\bm{U}$}}
\newcommand{\biX}{\mbox{$\bm{X}$}}
\newcommand{\biY}{\mbox{$\bm{Y}$}}
\newcommand{\biZ}{\mbox{$\bm{Z}$}}





\newcommand{\bA}{\mbox{\rm \bf A}}
\newcommand{\bB}{\mbox{\rm \bf B}}
\newcommand{\bC}{\mbox{\rm \bf C}}
\newcommand{\bD}{\mbox{\rm \bf D}}
\newcommand{\bE}{\mbox{\rm \bf E}}
\newcommand{\bF}{\mbox{\rm \bf F}}
\newcommand{\bG}{\mbox{\rm \bf G}}
\newcommand{\bH}{\mbox{\rm \bf H}}
\newcommand{\bI}{\mbox{\rm \bf I}}
\newcommand{\bJ}{\mbox{\rm \bf J}}
\newcommand{\bL}{\mbox{\rm \bf L}}
\newcommand{\bK}{\mbox{\rm \bf K}}
\newcommand{\bM}{\mbox{\rm \bf M}}
\newcommand{\bO}{\mbox{\rm \bf O}}
\newcommand{\bP}{\mbox{\rm \bf P}}
\newcommand{\bQ}{\mbox{\rm \bf Q}}
\newcommand{\bR}{\mbox{\rm \bf R}}
\newcommand{\bS}{\mbox{\rm \bf S}}
\newcommand{\bT}{\mbox{\rm \bf T}}
\newcommand{\bU}{\mbox{\rm \bf U}}
\newcommand{\bV}{\mbox{\rm \bf V}}
\newcommand{\bX}{\mbox{\rm \bf X}}
\newcommand{\bW}{\mbox{\rm \bf W}}
\newcommand{\bY}{\mbox{\rm \bf Y}}
\newcommand{\bZ}{\mbox{\rm \bf Z}}
\newcommand{\balpha}{\mbox{\boldmath $\alpha$}}
\newcommand{\bbeta}{\mbox{\boldmath $\beta$}}
\newcommand{\bepsilon}{\mbox{\boldmath $\epsilon$}}
\newcommand{\bgamma}{\mbox{\boldmath $\gamma$}}
\newcommand{\bdelta}{\mbox{\boldmath $\delta$}}
\newcommand{\boldeta}{\mbox{\boldmath $\eta$}}
\newcommand{\blambda}{\mbox{\boldmath $\lambda$}}
\newcommand{\bkappa}{\mbox{\boldmath $\kappa$}}
\newcommand{\bomega}{\mbox{\boldmath $\omega$}}
\newcommand{\bmu}{\mbox{\boldmath $\mu$}}
\newcommand{\bnu}{\mbox{\boldmath $\nu$}}
\newcommand{\bphi}{\mbox{\boldmath $\phi$}}
\newcommand{\bpi}{\mbox{\boldmath $\pi$}}
\newcommand{\bpsi}{\mbox{\boldmath $\psi$}}
\newcommand{\brho}{\mbox{\boldmath $\rho$}}
\newcommand{\bsigma}{\mbox{\boldmath $\sigma$}}
\newcommand{\btau}{\mbox{\boldmath $\tau$}}
\newcommand{\btheta}{\mbox{\boldmath $\theta$}}
\newcommand{\bvarepsilon}{\mbox{\boldmath $\varepsilon$}}
\newcommand{\bxi}{\mbox{\boldmath $\xi$}}
\newcommand{\bzeta}{\mbox{\boldmath $\zeta$}}
\newcommand{\bDelta}{\mbox{\boldmath $\Delta$}}
\newcommand{\bGamma}{\mbox{\boldmath $\Gamma $}}
\newcommand{\bLambda}{\mbox{\boldmath $\Lambda $}}
\newcommand{\bOmega}{\mbox{\boldmath $\Omega$}}
\newcommand{\bPhi}{\mbox{\boldmath $\Phi$}}
\newcommand{\bSigma}{\mbox{\boldmath $\Sigma$}}
\newcommand{\bTheta}{\mbox{\boldmath $\Theta$}}
\newcommand{\bXi}{\mbox{\boldmath $\Xi$}}



\newcommand{\bias}{ \mbox{\rm bias} }
\newcommand{\blockdiag}{ \mbox{\rm blockdiag} }
\newcommand{\diag}{ \mbox{\rm diag} }
\newcommand{\Diag}{ \mbox{\rm Diag} }
\newcommand{\range}{ \mbox{\rm range} }
\newcommand{\rank}{\mbox{\rm rank}}
\newcommand{\sd}{ \mbox{\rm SD} }
\newcommand{\SD}{ \mbox{\rm SD} }
\newcommand{\SE}{ \mbox{\rm SE} }
\newcommand{\se}{ \mbox{\rm SE} }
\newcommand{\qse}{ \mbox{\rm QSE} }  % QuasiSE
\newcommand{\QSE}{ \mbox{\rm QSE} }  % QuasiSE
\newcommand{\sgn}{ \mbox{\rm sgn} }
\newcommand{\sign}{ \mbox{\rm sign} }
\newcommand{\tr}{ \mbox{\rm trace} }
\newcommand{\trace}{ \mbox{\rm trace} }
\newcommand{\Cov}{ \mbox{\rm Cov} }
\newcommand{\Var}{ \mbox{\rm Var} }
\newcommand{\vvec}{ \mbox{\rm vec} }
\newcommand{\Corr}{ \mbox{\rm Corr} }




% zz these will have to be changed for VGAM
\newcommand{\GLIM}{{\sc glim}}
\newcommand{\GENSTAT}{{\sc genstat}}
\newcommand{\FORTRAN}{{\sc fortran}}
\newcommand{\C}{{\sc c}}

% 20090309
\newcommand{\pkg}[1]{\mbox{{\sf #1}}}

% zz added by me
%\newcommand{\VGAM}{{\sc vgam}}
 \newcommand{\VGAM}{\pkg{VGAM}}
 \newcommand{\VGAMdata}{\pkg{VGAMdata}}
 \newcommand{\SMARTPRED}{{\sc smartpred}}
%\newcommand{\VGAM}{\mbox{{\sc vgam}${\rm s}^2$}}

 \newcommand{\NULL}{\mbox{\tt NULL}}
 \newcommand{\NA}{\mbox{\tt NA}}
 \newcommand{\NAs}{{\mbox{\tt NA}s}}
 \newcommand{\FALSE}{\mbox{\tt FALSE}}
 \newcommand{\TRUE}{\mbox{\tt TRUE}}
 \newcommand{\tts}{\mbox{\tt s}}
 \newcommand{\ttsb}{\mbox{\tt s()}}
 \newcommand{\ttbs}{\mbox{\tt bs}}
 \newcommand{\ttbsb}{\mbox{\tt bs()}}
 \newcommand{\ttns}{\mbox{\tt ns}}
 \newcommand{\ttnsb}{\mbox{\tt ns()}}
 \newcommand{\ttpoly}{\mbox{\tt poly}}
 \newcommand{\ttpolyb}{\mbox{\tt poly()}}
 \newcommand{\ttscale}{\mbox{\tt scale}}
 \newcommand{\ttscaleb}{\mbox{\tt scale()}}

 \newcommand{\ttlm}{\mbox{\tt lm}}
 \newcommand{\ttlmb}{\mbox{\tt lm()}}
 \newcommand{\ttvlm}{\mbox{\tt vlm}}
 \newcommand{\ttvlmb}{\mbox{\tt vlm()}}
 \newcommand{\ttvglm}{\mbox{\tt vglm}}
 \newcommand{\ttvglmb}{\mbox{\tt vglm()}}
 \newcommand{\ttvgam}{\mbox{\tt vgam}}
 \newcommand{\ttvgamb}{\mbox{\tt vgam()}}
 \newcommand{\ttrrvglm}{\mbox{\tt rrvglm}}
 \newcommand{\ttrrvglmb}{\mbox{\tt rrvglm()}}
\newcommand{\ttgam}{\mbox{\tt gam}}
\newcommand{\ttgamb}{\mbox{\tt gam()}}
\newcommand{\ttglm}{\mbox{\tt glm}}
\newcommand{\ttglmb}{\mbox{\tt glm()}}
\newcommand{\ttglimb}{\mbox{\tt glim()}}

\newcommand{\ttlmbglmbgamb}{\mbox{{\tt lm()}/{\tt glm()}/{\tt gam()}}}
\newcommand{\ttglmbgamb}{\mbox{{\tt glm()}/{\tt gam()}}}
\newcommand{\ttvglmbvgamb}{\mbox{{\tt vglm()}/{\tt vgam()}}}


\newcommand{\R}{{\textsf{R}}}
\newcommand{\RR}{{\textsf{R}}}
\newcommand{\VSPLINE}{{\sc vspline}}      % zz added by me; should be as \VGAM
\newcommand{\YEESPLINE}{{\sc yee-spline}} % zz added by me; should be as \VGAM
\newcommand{\GAM}{{\sc gam}}
\newcommand{\GLM}{{\sc glm}}
\newcommand{\LM}{{\sc lm}}
\newcommand{\UNIX}{{\sc unix}}
\newcommand{\LINPACK}{{\sc linpack}}
\newcommand{\LAPACK}{{\sc lapack}}
\newcommand{\SPLUS}{{\textsf{S-PLUS}}}
\newcommand{\degrees}{\mbox{$^{\circ}$}}
\newcommand{\degreesC}{\mbox{$^{\circ}$C}}
\newcommand{\degreesF}{\mbox{$^{\circ}$F}}
\newcommand{\argmax}{\mbox{arg max}}
\newcommand{\argmin}{\mbox{arg min}}
\newcommand{\Unif}{\mbox{Unif}}
\newcommand{\Beta}{\mbox{Beta}}
% \newcommand{\swea}[1]{\mbox{\textsl{\texttt{#1}}}}
% \newcommand{\sweat}[1]{\mbox{\textsl{\texttt{#1}}}}

\newcommand{\swea}[1]{\mbox{{\texttt{#1}}}}
\newcommand{\sweat}[1]{\mbox{{\texttt{#1}}}}


%\newcommand{\dferr}{\mbox{{\em df}$^{\rm \ err}$}}
%\newcommand{\dfe}{\mbox{{\em dfe}}}


% ,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,
% 20111005; from Trevor Hastie, fhat.sty, etc.

\newcommand{\half}{\frac{1}{2}}
\newcommand{\Co}[1]{{\small\tt #1}}
%\def\R{{\mathrm{I}\!\mathrm{R}}}
%\usepackage{exercise}
%\numberexercises{chapter}
\def\Prob{\mbox{\rm Pr}}
\def\Pr{\mbox{\rm Pr}}


%%\definecolor{Purple}{cmyk}{0.333,0.867,0.0,0.059}  % http://web.forret.com/tools/color 20140819
%\definecolor{brightblue}{cmyk}{1,.5,0,0}
%\definecolor{goldenrod}{cmyk}{0,.2,1,0}
%\definecolor{cborange}{rgb}{0.9,0.62,0.0}%cb.cols
%\definecolor{cbblue}{rgb}{0.34,0.71,0.91}%cb.cols
%%\definecolor{cborange}{rgb}{1.0000000, 0.5725490, 0.20000000}%cbmit.cols
%%\definecolor{cbblue}{rgb}{0.1607843, 0.8156863, 0.81568627}%cbmit.cols





%  %20120111; this is definitive in this file.
%  %20120111; convert the above colours to rgb so that R can do it.
%  % Use http://www.usq.edu.au/users/grantd/WORK/216color/ConvertRGB-CMYK-Grey.htm
%  % round(100 * c(1,.5,0,0) / sum(c(1,.5,0,0)), dig = 2)
%  % 66.67 33.33  0  0
%  \definecolor{Brightblue}{rgb}{85,170,255}
%  \definecolor{Brightblue}"#6699FF" % web-safe
%  \definecolor{Brightblue}"#55AAFF"
%
%  % round(100 * c(0,.2,1,0) / sum(c(0,.2,1,0)), dig = 2)
%  % 0.00 16.67 83.33  0.00
%  \definecolor{Goldenrod}{rgb}{255,212,43}
%  \definecolor{Goldenrod}"#FFCC33"  % web-safe
%  \definecolor{Goldenrod}"#FFD42B"
%
%  % round(255 * c(0.9, 0.62, 0))
%  % 230 158   0
%  \definecolor{Cborange}"#E69E00"  %
%  \definecolor{Cborange}"#FF9900"  % web-safe
%
%  % round(255 * c(0.34, 0.71, 0.91))
%  % 87 181 232
%  \definecolor{Cbblue}"#57B5E8"  %
%  \definecolor{Cbblue}"#66CCFF"  % web-safe






%20120111; this solution is suboptimal. Better to edit svmono.cls.
%\newcommand{\mysection}[1]{\color{brightblue} \section{#1}}
%\newcommand{\mysubsection}[1]{\color{brightblue} \subsection{#1}}
%\newcommand{\mysubsubsection}[1]{\color{brightblue} \subsubsection{#1}}
%\newcommand{\mysection*}[1]{\color{brightblue} \section*{#1}}
%\newcommand{\mysubsection*}[1]{\color{brightblue} \subsection*{#1}}
%\newcommand{\mysubsubsection*}[1]{\color{brightblue} \subsubsection*{#1}}



% ,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,
% 20110325; for compatibility with Beamer slides, e.g., from Melbourne

\newcommand{\rformula}[1]{{#1}}

\newcommand{\RSS}{\mbox{\rm ResSS}}
\newcommand{\ResSS}{\mbox{\rm ResSS}}
\newcommand{\Dollar}{{\$}}


% ,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,
% 20130809; i am commenting out this block of code. It messes
% up knitr.

%% 20110330; for compatibility with doc.tex
%
%\def\alltt{\trivlist \item[]\if@minipage\else\vskip\parskip\fi
%\leftskip\@totalleftmargin\rightskip\z@
%\parindent\z@\parfillskip\@flushglue\parskip\z@
%\@tempswafalse \def\par{\if@tempswa\hbox{}\fi\@tempswatrue\@@par}
%\obeylines \small \tt \catcode``=13 \@noligs \let\do\@makeother \docspecials
% \frenchspacing\@vobeyspaces}
%
%\let\endalltt=\endtrivlist
%
%\newenvironment{Example}{\begin{list}{}{\setlength{\leftmargin}{\parindent}}\item
%\begin{alltt}}{\end{alltt}\end{list}}



% ,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,
% 20120723; for compatibility with workshops and beamer etc.

\newcommand{\rcoderm}[1]{{\textrm{#1}}}
\newcommand{\rcodett}[1]{{\texttt{#1}}}
\newcommand{\rcodesf}[1]{{\textsf{#1}}}
\newcommand{\rcodeit}[1]{{\textit{#1}}}
\newcommand{\rcodebf}[1]{{\textbf{#1}}}


% ,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,
% 20131125; more macros....
\newcommand{\OIM}{\mbox{{\boldmath ${\cal I}$}${}_{\mathrm{O}}$}}   % bold \cI or \bcalI
\newcommand{\EIM}{\mbox{{\boldmath ${\cal I}$}${}_{\mathrm{E}}$}}   % bold \cI or \bcalI
\newcommand{\OIMinv}{\mbox{{\boldmath ${\cal I}$}${}_{\mathrm{O}}^{-1}$}}
\newcommand{\EIMinv}{\mbox{{\boldmath ${\cal I}$}${}_{\mathrm{E}}^{-1}$}}
\newcommand{\OIMsup}[1]{\mbox{{\boldmath ${\cal I}$}${}_{\mathrm{O}}^{#1}$}}
\newcommand{\EIMsup}[1]{\mbox{{\boldmath ${\cal I}$}${}_{\mathrm{E}}^{#1}$}}


% For one observation...
\newcommand{\OIMone}{\mbox{{\boldmath ${\cal I}$}${}_{\mathrm{O}1}$}}   % bold \cI or \bcalI
\newcommand{\EIMone}{\mbox{{\boldmath ${\cal I}$}${}_{\mathrm{E}1}$}}   % bold \cI or \bcalI
\newcommand{\OIMinvone}{\mbox{{\boldmath ${\cal I}$}${}_{\mathrm{O}1}^{-1}$}}
\newcommand{\EIMinvone}{\mbox{{\boldmath ${\cal I}$}${}_{\mathrm{E}1}^{-1}$}}

\newcommand{\EIMsub}[1]{\mbox{{\boldmath ${\cal I}$}${}_{\mathrm{E},#1}^{}$}}

% 20141021; more macros....
\newcommand{\bcalA}{\mbox{{\boldmath ${\cal A}$}}}   %
\newcommand{\bcalB}{\mbox{{\boldmath ${\cal B}$}}}   %
\newcommand{\bcalC}{\mbox{{\boldmath ${\cal C}$}}}   %
\newcommand{\bcalH}{\mbox{{\boldmath ${\cal H}$}}}   %
\newcommand{\bcalP}{\mbox{{\boldmath ${\cal P}$}}}   %
\newcommand{\bcalU}{\mbox{{\boldmath ${\cal U}$}}}   %

% 20150102; more macros....
\newcommand{\sdee}{\mbox{\scriptsize {$d$}}}   % $d$, this is the number of raw covariates/terms
\newcommand{\dee}{\mbox{$d$}}   % $d$, this is the number of raw covariates/terms
\newcommand{\sbH}{\mbox{\scriptsize \rm \bf H}}


% 20150115; more macros....
% \underset{x}{\operatorname{argmax}}
% \DeclareMathOperator*{\argmin}{arg\,min}


% ,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,
% 20150611; more macros....


\newcommand{\forthereader}{\mbox{\rm FOR\ THE\ READER\ TO\ DO}}
\newcommand{\fixupone}[1]{{\textbf{#1}}}

% ,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,



% ,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,






% ,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,


% ,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,,



